Deep combinatorial optimisation for optimal stopping time problems : application to swing options pricing

A new method for stochastic control based on neural networks and using randomisation of discrete random variables is proposed and applied to optimal stopping time problems. The method models directly the policy and does not need the derivation of a dynamic programming principle nor a backward stochastic differential equation. Unlike continuous optimization where automatic differentiation is used directly, we propose a likelihood ratio method for gradient computation. Numerical tests are done on the pricing of American and swing options. The proposed algorithm succeeds in pricing high dimensional American and swing options in a reasonable computation time, which is not possible with classical algorithms.

==> 4_impulse.tex <==
\section{Extension to stochastic impulse control}
\label{sec:impulse}
In this section we present how the algorithm of Section \ref{sec:optimalstoppingalgorithm} can be combined to the method described in \cite{fecamp2019risk} for impulse control problems. Impulse control has a lot of applications in economics and finance (real options valuation in energy markets, and optimal order execution in illiquid markets...). In Section \ref{sec:numericalfixed}, we apply the algorithm to an option hedging under fixed transaction costs. \\ 


\medskip
An impulse control is a sequence $(\tau, \zeta) = (\tau_i, \zeta_i)_{i \geq 1}$ with $(\tau_i)$ a sequence of increasing $\mathbb{F}$ stopping times and $(\zeta_i)_{i \geq 1}$ a sequence of $(\mathcal{F}_{\tau_i})_ {i \geq 1}$-measurable random variables taking values in $E \subset \mathbb{R}^d$. Let $\mathcal{A}$ the set of impulse control. A stochastic impulse control problem is the optimisation problem 
\begin{equation} \label{eq:impulsecontinuous}
   \underset{(\tau, \zeta) \in \mathcal{A}}{\sup} \mathbb{E}_\mathbb{P}(f(\tau, \zeta, X))
\end{equation}
with $X$ the solution of \eqref{sde}. As for the optimal stopping time problems, the impulse control problems can be associated to a BSDE or to a quasi-variationnal inequality, see \cite{kharroubi10} and can only be solved numerically most of the time.


We consider the  discretisation of problem  \eqref{eq:impulsecontinuous} and we search for
\[
   \underset{(\tau, \zeta) \in \mathcal{A}^N}{\sup}  \mathbb{E}_\mathbb{P}(f(\tau, \zeta, X))
\]
where $\mathcal{A}^N \subset \mathcal{A}$ contains the control with $\tau$ taking values in a discrete set $\mathcal{D}_N$. This problem is equivalent to 
\begin{equation} \label{impulsediscrete}
    \underset{(Y, Z)}{\sup}  \mathbb{E}_\mathbb{P}(f_N(Y, Z, X))
\end{equation}
 where $(Y_i, Z_i)_{i=0,\ldots,N}$ is a sequence of  $(\mathcal{F}_{t_i})_{i=0,\ldots,N}$-measurable random variables with $Y_i$ taking values in $\{0,1\}$ and $Z_i$ taking values in $E$.
 
 
\begin{remark}
More generally, the process $X$ can depend on the control if jumps are present in its dynamic but this case is not considered here. 
\end{remark}


\subsection{Algorithm extension to impulse control}
\label{sec:algoimpulse}

%Our algorithm allows to solve the case where $Z_i = 1$ for all $i = 1,\ldots,N$ whereas the algorithm of \cite{fecamp2019risk} can only solve the case where $l = N$, $Y_i = 1$ for $i = 1,\ldots,N$. One neural network is considered to train blablabla

$Z$ is a continuous control and can be optimised as done in \cite{fecamp2019risk}. A neural network $\mathbb{NN}_Z$ with vector of parameters $\theta_{Z}$ outputs the optimal continuous control:
\[Z_{t_i} = \mathbb{NN}_{Z}(t_i, X_{t_i}, \theta_{Z})\]
with $\theta_{Z} \in \Theta_Z$ the set in which the bias and weights of $\mathbb{NN}_{Z}$ lie. $\mathbb{NN}_{Z}$ is chosen as a Recurrent Neural Network, see Section  \ref{sec:architectureimpulse}, but for ease of notation, the dependence with the memory of the neural network is omitted.


$Y$ is again supposed to be Bernoulli distributed with a probability parameterised by a neural network $\mathbb{NN}_{Y}$ with vector of parameters $\theta_Y$. Omitting the constraints (which can be easily added as in Equation \eqref{eq:paramNNwithconstraints}), the probability is parameterised as in Equation \eqref{eq:paramNN}:
\begin{equation}
\label{eq:paramNNwithinput}
\mathbb{P}(Y_j = 1 | X_{t_j}) = expit\left( C \times tanh\left(\mathbb{NN}_Y(t_j, X_{t_j}, \theta_{Y})), \theta_Y\right)\right), \; j=0,\ldots,N,
\end{equation}
with $\theta_{Y} \in \Theta_Y$ the set in which the bias and weights of $\mathbb{NN}_Y$ lie. 


%Let $\Theta_\Delta$ (resp. $\Theta_Y$) be the sets in which the bias and weights of $\mathbb{NN}_\Delta$ (resp.$\mathbb{NN}_\tau$) lies. Compared to \ref{sec:optimalstoppingalgorithm} a new feature is added to $\mathbb{NN}_\tau$:
%\begin{eqnarray}
%\mathbb{NN}_{\Delta} : \mathbb{R} \times \mathbb{R}^d \times \Theta_\Delta  &\rightarrow& \mathbb{R}^d \\
%(t_i, X_{t_i}, \theta) &\mapsto& Z_{t_i}^\theta,\\ 
%\mathbb{NN}_{\tau} : \mathbb{R} \times \mathbb{R}^d \times \mathbb{R}^d  \times \Theta_\tau  &\rightarrow &\{0, 1\} \\
%(t_i, X_{t_i}, \Delta_{t_i}, \theta)& \mapsto& %\mathbb{P}_{\theta}(\tau = 1).
%\end{eqnarray}
%We  search for the optimal $\theta_{\Delta}, \theta_Y:
%\begin{eqnarray}
%\hat{\theta}_\zeta, \hat{\theta}_\tau \in \argmax_{\theta_\zeta \in \Theta_\zeta, \theta_\tau \in \Theta_\tau } \mathbb{E}_\mathbb{P}\left( g(Y^{\theta_\zeta}, Z^{\theta_\tau}, X^N)\right)
%\end{eqnarray}
Algorithm  \ref{algo:algoimpulse} finds the optimal parameters of the neural networks. The algorithm is quite similar to Algorithm \ref{algo:algoGlobal} except there is a gradient descent over the parameters $\theta_{Z}$. The computation of this gradient is easily done using backpropagation. In Algorithm \ref{algo:algoimpulse}, the two gradients are concatenated in order to have one gradient updated with one learning rate: it is possible (and it is used in some of the results hereafter) to consider two different learning rates and to update each gradient separately.

\begin{algorithm}[H]

\begin{algorithmic}[1]
 \State $\alpha_0$ : Initial stepsize
 \State $r_{\alpha} \in [0,1]$: Stepsize reduction
 \State $\beta_1$, $\beta_2\in[0,1]:$ Exponential decay rates for the moment estimates,
 \State $N_{iter}:$ number of iterations
 \State $N_{batch}:$ number of simulations at each gradient descent iteration (batch size)
\State {\color{blue} $\theta_{0} = (\theta_{Z,0}, \theta_{Y,0})$ randomly chosen}
\State $m_0 \leftarrow 0 $
\State $v_0 \leftarrow 0$ 
\State $i_{iter} \leftarrow 0 $
\For{$i_{iter}=0\ldots N_{Iter}$}
\For{$u=0 \ldots N$}
\State $X_u \leftarrow N_{batch}$ samples simulations of $X_{t_u}$
\State {\color{blue} $\Delta_u \leftarrow \mathbb{NN}_{Z}(t_u, X_{t_u}, \theta_{Z, iter})$.}
\State $Y_u \leftarrow N_{batch}$ of a Bernouilli r.v. with parameter $expit\left( C \times tanh\left(\mathbb{NN}_Y(t_u, X_u,   \theta_{Y,i_{iter}})\right)\right)$ 
\EndFor
\State $i_{iter} \leftarrow i_{iter} +1 $
\State {\color{blue}
$g_{i_{iter}, Z} \leftarrow \nabla_{\theta_{Z}}\frac{1}{N_{batch}} \sum_{n=1}^{N_{batch}} f_N(Y^n, Z^n, X^n) $
(get objective function gradient w.r.t $\theta_{Z}$)}
\State 
\[
g_{i_{iter}, Y} \leftarrow \frac{1}{N_{batch}} \sum_{n=1}^{N_{batch}} f_N(Y^n, Z^n, X^n)
\left(\sum_{u=0}^{N} \nabla_{\theta_Y } \log\left(expit\left( C \times tanh \left(\mathbb{NN}_Y(t_u, X^n_{t_u}, \theta_{Y, i_{iter}-1})\right)\right) \right)\right)
\]
(get objective function gradient w.r.t $\theta_Y$)
\State {\color{blue} $g_{i_{iter}} \leftarrow (g_{i_{iter}, Z}, g_{i_{iter}, Y})$ (concatenate gradients)}
\State  $m_{i_{iter}} \leftarrow m_{{i_{iter-1}}} + (1-\beta_1) g_{i_{iter}}$ (update biased first moment estimate) 
\State $v_{i_{iter}} \leftarrow \beta_2 v_{{i_{iter-1}}} + (1-\beta_2) g_{i_{iter}} ^2$ (update biased second raw moment estimate)
\State $\hat{m}_{i_{iter}}  \leftarrow \frac{m_{i_{iter}}}{1-\beta_1^{i_{iter}}}$ (computes bias-corrected first moment estimate ($\beta_1^{i_{iter}}$ stands for $\beta_1$ to the power of ${i_{iter}}$)) 
\State $\hat{v}_{i_{iter}}  \leftarrow \frac{v_{i_{iter}}}{1-\beta_2^{i_{iter}}}$ (computes bias-corrected second raw moment estimate ($\beta_2^{i_{iter}}$ stands for $\beta_1$ to the power of ${i_{iter}}$))
\State $\theta_{i_{iter}} \leftarrow \theta_{i_{iter}-1} - \alpha_{iter} \hat{m}_{i_{iter}} /(\sqrt{\hat{v}_{i_{iter}}}+\epsilon )$ (update parameters)
\State $\alpha_{i_{iter}} \leftarrow r_{\alpha} \alpha_{i_{iter}-1} $ (update stepsize)
\EndFor
\end{algorithmic}
\caption{Algorithm for impulse control problems. Main differences with Algorithm \ref{algo:algoGlobal} are in blue.}
\label{algo:algoimpulse}
\end{algorithm}


\subsection{Architecture of the neural networks}
\label{sec:architectureimpulse}
We propose to follow \cite{fecamp2019risk} but we use two recurrent neural networks, one for $\mathbb{NN}_Z$ and another one for $\mathbb{NN}_Y$. The recurrent cells are LSTM cells \cite{article:lstm} among which a series of feedforward layers are placed (see Figure \ref{fig:architectureimpulse}). One could give as inputs of $\mathbb{NN}_Y$ the outputs of $\mathbb{NN}_Z$ but from our tests it appears that it does not improve the results.
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\textwidth]{./img/inpulse_architecture.jpg}
    \caption{Architecture of the graph for impulse control. First control and premium are variables that are trained outside neural networks.}
    \label{fig:architectureimpulse}
\end{figure}

\subsection{Numerical results: application to fixed transaction costs}
\label{sec:numericalfixed}

In this section we consider the problem of hedging an European style option paying $g(X_T)$ under fixed transaction costs: at each date $t_i, i \in \{0,\ldots,N\}$ and for each asset $k \in \{1,\ldots,d\}$, the portfolio manager pays a constant fee $c^k_i$ that does not depend on the volume of underlying $k$ that is purchased or sold (given that the volume is not null).  We search for an impulse control $(Y, Z)$ with $Y_i = 1$ if there is an hedge at time $t_i, i \in \{0,\ldots, N\}$ and $Z^k_i$ corresponds to the quantity of asset $k, k \in \{1,\ldots,d\}$ to buy or sell at time $t_i$. Let us consider the self-financing portfolio with value at time $t_j, j \in \{0, \ldots,N\},$
\begin{equation} \label{eq:portfolio}
\Pi_{t_j} = P_0 + \sum_{k=1}^d \sum_{i = 1}^{j} \Delta^k_{i-1} (X^k_{t_i}-X^k_{t_{i-1}})
\end{equation}
where $\Delta_i$ corresponds to the amount of asset held at time $t_i$, $P_0$ corresponds to the option premium and where 
\[
\left\{
\begin{array}{ll}
     \Delta_0 = Z_0  \\
     \Delta_i = \Delta_{i-1} + Y_i Z_i, \; i = 1,\ldots,N-1.
\end{array}
\right.
\]
The last control $(Y_N, Z_N)$ does not appear in the replication portfolio and nor in the optimisation problem. The transaction costs paid until time $t_j$, $j \in \{0,\ldots,N\}$, generated by the strategy is equal to 
\begin{equation}
    C_{t_j}  =\sum_{i = 0}^{j-1} \sum_{k=1}^d  Y_{i} c_j^k. \label{eq:fixedcosts} 
\end{equation}
One searches for an impulse control $(Y, Z)$ and an initial premium $P_0$ that minimises the moment-based criteria: 
\begin{eqnarray} \label{eq:meanvariance}
L_f(X, Y, Z) & = & \beta \Ebb_{\mathbb{P}}(C_T) + (1 - \beta) \Ebb_{\mathbb{P}}(E_T^2) 
\end{eqnarray}
where 
\begin{equation} \label{eq:hedgedportfolio}
E_T =\Pi_T - g(X_T) 
\end{equation}
is the replication error and $\beta\in[0,1]$ quantifies the trade-off between the average costs $\Ebb_{\mathbb{P}}(C_T)$ ad the $L^2$ loss $\Ebb_{\mathbb{P}}(E_T^2)$.
One could consider different risk criteria as in \cite{fecamp2019risk} but the mean-variance choice is convenient for comparison to usual stochastic control methods as a dynamic stochastic programming equation can be derived. Practitioners prefer to use the homogeneous criterion $\beta \Ebb_{\mathbb{P}}(C_T) + (1 - \beta) \sqrt{\Ebb_{\mathbb{P}}(E_T^2) }$ which can be addressed by Algorithm \ref{algo:algoimpulse} but not by dynamic programming approaches. 

\subsubsection{European call option}
\label{sec:callimpulse}
In this section, we hedge an European call option (dimension 1, payoff $(x-K)^+$) in the Black-Scholes framework ($X$ is the solution of \eqref{sde} with $\mu(t,x) = 0$ and $\sigma(t,x) = \sigma x$) with  
\begin{itemize}
    \item Case 1: $X_0 =1, K = 1, T = 1, \sigma = 25\%$, $c_j = c = 0.001$ for every $j \in \{0,\ldots,N\}$, $\beta = 0.25$, and $N= 10$, 
   \item  Case 2: $X_0 =1, K = 1, T = 2, \sigma = 25\%$, $c_j = c = 0.0005$ for every $j \in \{0,\ldots,N\}$, $\beta = 0.25$, $N=20$.  
\end{itemize}
The hedging dates belong to the regular grid $\mathcal{D}_N = \{\frac{i}{N}, \; i=0, \ldots, N\}$. To hedge those options, let us consider Algorithm \ref{algo:algoimpulse} with a batch size of $N_{batch} = 5,000$, a test set size of 50,000, a validation set size of 100,000, an initial learning rate of $\alpha_0 = 0.001$, a decay of $r_{\alpha} = 0.98^{1/100}$ (only for the neural networks associated with $Y$), $N_{iter} = 20,000$ iterations, a LSTM cell with 60 units followed by 3 layers of 20 neurons for $\mathbb{NN}_Y$ and a LSTM cell with 50 unis followed by 3 layers of 10 neurons for $\mathbb{NN}_Z$. $P_0$ is a trainable variable that is optimised. We compare Algorithm \ref{algo:algoimpulse} to three strategies:
\begin{itemize}
\item The Black-Scholes strategy which consists in hedge at each time step with the Black-Scholes delta. This strategy is naive as it does not take into account the transaction costs. $P_0$ is equal to $\mathbb{E}(g(X_t))$.
\item The strategy described in \cite{whalley1993counting}. In this latter paper, the cost function is the exponential utility function defined (with the notations defined in  \eqref{eq:portfolio}, \eqref{eq:hedgedportfolio} and \eqref{eq:fixedcosts}) by:
\begin{eqnarray}
U_\gamma(\delta, q)  & = &  \Ebb_{\mathbb{P}}\left(e^{- \gamma (C_T + E_T)}\right).  \label{eq:utility}
\end{eqnarray}
 The strategy results in a traditional Black-Scholes strategy with boundaries. Assuming zero interest rate,  boundaries are given by $\Delta_{BS, t} \pm H_t(\gamma)$ where %http://users.ox.ac.uk/~ofrcinfo/file_links/mf_papers/1999mf17.pdf
\begin{eqnarray}
H_{t}(\gamma)  & = &\left(\frac{12 c (\Gamma_{BS,t}) ^2}{\gamma} \right)^\frac{1}{4} 
\end{eqnarray}
and where $\Delta_{BS,t}$ and $\Gamma_{BS,t}$ are the traditional Black-Scholes $\Delta$ and $\Gamma$ at time $t$. The strategy is then the following:
\[
\Delta_{0} =  \begin{cases} \Delta_{BS, t_0} & \mbox{if } | \Delta_{BS, t_0} | \geq H_{t_0}(\gamma) \\ 
0 & \mbox{otherwise }  \end{cases}
,
\]
\[
\Delta_{j} =  \begin{cases} \Delta_{BS, t_j} & \mbox{if } | \Delta_{BS, t_j} - \Delta_{j-1} | \geq H_{t_j}(\gamma) \\ 
\Delta_{j-1} & \mbox{otherwise }  \end{cases}, \;j = 1, \ldots, N-1
\]
and the optimal premium is given by $P_0 = \mathbb{E}_{\mathbb{P}}(g(X_T))$.
Despite its desirable properties, exponential utility cost function is difficult to deal with when it is used in a numerical resolution algorithm and one prefers the criteria \eqref{eq:meanvariance}. As we do not know the equivalence between the risk aversion $\gamma$ for the criteria \eqref{eq:utility} and the one for the criteria \eqref{eq:meanvariance} $\beta$, we consider all the strategies given by \cite{whalley1993counting} varying $\gamma$ and choose the one minimising \eqref{eq:meanvariance}. In practice, we make $\gamma$ vary on a regular grid with 1000 points between 0 and 30.
\item A dynamic programming approach, solved with the library \cite{gevret18}.
\end{itemize}


In Figure \ref{fig:wwvsnn}, the losses between a Black-Scholes strategy that does not take into account costs, the neural network strategy computed with Algorithm \ref{algo:algoimpulse} and the Whalley-Wilmott strategy for multiple risk aversion are compared. The optimal risk aversion with respect to criteria \eqref{eq:meanvariance} is equal to 22.82 for 10 dates and 20.29 for 20 dates. Results are given in Table \ref{tab:fixed_comparison}. The Whalley-Wilmott, Dynamic programming and Algorithm \ref{algo:algoimpulse} improve a lot the loss compared to the Black-Scholes strategy in both cases. Hedging positions from 4 simulations and the different strategies are given in Figure \ref{fig:delta10} for case 1 and in Figure \ref{fig:delta20} for case 2. We can see the intuitive behaviour consisting in waiting for the transaction-cost-free delta to change sufficiently before doing anything. When 10 hedging dates are considered, the three strategies give similar losses. However, the hedging error and costs are not the same: Dynamic Programming and Algorithm \ref{algo:algoimpulse} hedge more than Whalley-Wilmott. We can see that Algorithm \ref{algo:algoimpulse} performs well. Considering 20 dates, the neural network is sligthly sub optimal: on Figure \ref{fig:delta20}, one can see that the continuous control is not perfect. However we notice that the loss is still decreasing after 20,000 iterations but very slowly. Computation times are comparable between Dynamic programming and Algorithm \ref{algo:algoimpulse}, see \ref{tab:timefixed_comparison}: a high precision is needed in the regression for the Dynamic programming algorithm due to the lack of smoothness of the problem around 0 while the convergence requires a batch size sufficiently high and 20,000 iterations for Algorithm \ref{algo:algoimpulse}. However, one expects for Algorithm \ref{algo:algoimpulse} to be more robust when dimension increases. 

\begin{figure}
    \centering
    \includegraphics[width = 0.45\textwidth]{img/whalley_wilmott_NN_ATM_10_dates.jpeg}
    \includegraphics[width = 0.45\textwidth]{img/whalley_wilmott_NN_ATM_20_dates.jpeg}
    \caption{Comparison of losses between Whalley-Wilmott, traditional Black-Scholes and Algorithm \ref{algo:algoimpulse} with various risk aversion in \eqref{eq:utility}. Left: Case 1 (10 dates); Right: Case 2 (20 dates) (Neural network stands for Algorithm \ref{algo:algoimpulse}).}
    \label{fig:wwvsnn}
\end{figure}

\begin{table}
    \centering
\begin{tabular}{|c|c|c|c|c|} \hline 
  Case     &  Black-Scholes & Whalley-Wilmott & Dynamic programming & Algorithm \ref{algo:algoimpulse}  \\ \hline 
10 dates & 0.00302 (0.01/0.00069)& 0.00169 (0.0036/0.0011) & 0.00169 (0.0030/0.0.0013) &0.00170 (0.0032/0.0012)\\  \hline 
20 dates & 0.00277 (0.01/0.00036) & 0.00114  (0.0027/0.0006)
 & 0.00119 (0.0021/0.0009) &  0.00134 (0.0024/0.001)\\ \hline 
\end{tabular}
    \caption{Loss (Cost/$L^2$ loss) comparison between Whalley-Wimott strategy, dynamic programming and Algorithm \ref{algo:algoimpulse} on a call option with fixed transaction costs.}
    \label{tab:fixed_comparison}
\end{table}

\begin{table}[ht]
\centering
\begin{tabular}{|c|c|c|} \hline 
 Case & Stochastic control & Algorithm \ref{algo:algoimpulse}  \\ \hline 
10 dates & 2928 & 4004\\  \hline 
20 dates  & 14310 & 9423 \\ \hline 
\end{tabular}
    \caption{Time (in seconds) comparison between dynamic programming and Algorithm \ref{algo:algoimpulse} on a one-dimensional call option with fixed transaction costs.}
    \label{tab:timefixed_comparison}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width = 0.49\textwidth]{img/delta_NN_ATM_10_dates_sim1.jpeg}
    \includegraphics[width = 0.49\textwidth]{img/delta_NN_ATM_10_dates_sim2.jpeg}
    \includegraphics[width = 0.49\textwidth]{img/delta_NN_ATM_10_dates_sim3.jpeg}
    \includegraphics[width = 0.49\textwidth]{img/delta_NN_ATM_10_dates_sim4.jpeg}
    \caption{Comparison of bought quantities between Black-Scholes, Whalley-Wilmott, Dynamic programming and Algorithm \ref{algo:algoimpulse} for case 1 (Neural network stands for Algorithm \ref{algo:algoimpulse}).}
    \label{fig:delta10}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width = 0.49\textwidth]{img/delta_NN_ATM_20_dates_sim1.jpeg}
    \includegraphics[width = 0.49\textwidth]{img/delta_NN_ATM_20_dates_sim2.jpeg}
    \includegraphics[width = 0.49\textwidth]{img/delta_NN_ATM_20_dates_sim3.jpeg}
    \includegraphics[width = 0.49\textwidth]{img/delta_NN_ATM_20_dates_sim4.jpeg}
    \caption{Comparison of bought quantities between Black-Scholes, Whalley-Wilmott, Dynamic programming and Algorithm \ref{algo:algoimpulse} for case 2 (Neural network stands for Algorithm \ref{algo:algoimpulse}).}
    \label{fig:delta20}
\end{figure}

\subsubsection{3-dimensional spread option}
\label{sec:3Dimpulse}
We consider the hedging of the spread option on $N = 10$ dates with payoff
\[
(X_{1,T} - \frac{1}{2}(X_{2,T} + X_{3,T}) - K)^+
\]
where
\[dX_{i,t}= \sigma_i X_{i,t} dW_{i,t}, t \in \left[0,T\right]\; i = 1,\ldots,3,\]
$W$ is a multivariate Brownian motion with correlation matrix $$\begin{pmatrix} 
1 & 0.3 & 0.6  \\ 
0.3 & 1 & 0.2  \\
0.6 & 0.2 & 1
\end{pmatrix},$$
$(\sigma_1, \sigma_2, \sigma_3) = (0.25, 0.1, 0.1)$, $(X_{1,0}, X_{2,0}, X_{3,0}) = (1, 0.6, 0.6)$, $K = 0.4$, $T = 1$. The time mesh is $\mathcal{D}_N = \{\frac{i}{N}, \; i=0, \ldots, N\}$, the costs are given by $(c_j^1, c_j^2, c_j^3) = (0.002, 0.001, 0.0)$ for every $j \in \{0,\ldots,N\}$ and $\beta = 0.1$.

%\begin{enumerate}
%    \item One-cost-for-each: We just pay a fee on the future we trade. In this situation as the fee related to $X_3$ is lower than the fee related $X_1$, we expect to trade more often $X_3$ than $X_1$. This model the situation of paying a fee on three different markets. 
%    \item One-cost-for-all: 
%\end{enumerate}
%\paragraph{One-cost-for-each}
%In Table \ref{tab:3marketonecostforeach} the loss is compared between a stochastic control approach and Algorithm \ref{algo:algoimpulse}. Figure \ref{fig:delta3marketonecostforeach} shows the delta for 3 different simulations and the loss obtained after 10 000 iterations. One can see that the first underlying is traded less often than the two others that have lower transaction costs. 
%\begin{table}[ht]
%    \centering
%\begin{tabular}{|c|c|c|} \hline 
%& Loss & Time (s) \\ \hline 
%Algorithm \ref{algo:algoimpulse}  & 0.002294439  & \\ \hline 
%Stochastic control  & x & x \\ \hline
%\end{tabular}
%    \caption{Loss and time consumption for the hedging of a 3 markets spread in the one-cost-for-each case}
%    \label{tab:3marketonecostforeach}
%\end{table}

%\begin{figure}[ht]
%    \centering
 %   \includegraphics[width=0.49\textwidth]{img/delta_spread1.jpeg}
 %   \includegraphics[width=0.49\textwidth]{img/delta_spread2.jpeg}
 %   \includegraphics[width=0.49\textwidth]{img/delta_spread3.jpeg}
 %   \includegraphics[width=0.49\textwidth]{img/loss_spread.jpeg}
%    \caption{Delta for the spread option and associated loss estimated over the test set for the one-for-each situation}
%    \label{fig:delta3marketonecostforeach}
%\end{figure}
In Table \ref{tab:3marketonecostforall} the loss induced by Algorithm \ref{algo:algoimpulse} is compared to a naive strategy ignoring fixed transaction costs and computed using algorithm in \cite{fecamp2019risk}. Hyperparameters for Algorithm \ref{algo:algoimpulse} are: a LSTM cell of 50 unis followed by 3 layers of 10 neurons for $\mathbb{NN}_Z$, a LSTM cell of 60 units followed by 3 layers of 30 neurons for $\mathbb{NN}_Y$, batch size of 8,000, test size of 50,000, validation size of 100,000, $N_{iter} = 10,000$ iterations and an initial learning rate $\alpha$ equals to 0.001 and step size reduction $r_{\alpha} = 0.98^{1/100}$ (only for $mathbb{NN}_{Y}$). The use of Algorithm \ref{algo:algoimpulse} decreases global loss by 25\% as it hedges itself 2.06 times in average instead of the 10 times in the naive strategy.  \\ 
In this case, and due to the curse of dimensionality, stochastic control tools need hours on a cluster whereas our methodology runs on a personal laptop in one hour. Moreover, speed would be increased if a GPU would have been used. \\ 
Figure \ref{fig:deltaspread} shows the delta for 4 different simulations and compare the two strategies. 
\begin{table}[ht]
    \centering
\begin{tabular}{|c|c|} \hline 
& Loss \\ \hline 
Algorithm \ref{algo:algoimpulse}  & 0.00268 (0.00637/0.00227) \\ \hline 
Transaction costs free strategy  & 0.00356 (0.03/0.000629)  \\ \hline
\end{tabular}
      \caption{Loss (Cost/$L^2$ loss) for the hedging of a 3 markets spread.}
    \label{tab:3marketonecostforall}
\end{table}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{img/delta_spread_one_for_all1.jpeg}
    \includegraphics[width=0.45\textwidth]{img/delta_spread_one_for_all2.jpeg}
    \includegraphics[width=0.45\textwidth]{img/delta_spread_one_for_all3.jpeg}
    \includegraphics[width=0.45\textwidth]{img/delta_spread_one_for_all4.jpeg}
    \caption{Examples of delta for the spread option. Solid lines correspond to the strategy outputted by Algorithm \ref{algo:algoimpulse} and dotted lines to the costs free strategy.} 
    \label{fig:deltaspread}
\end{figure}

Algorithm \ref{algo:algoimpulse} extends Algorithm \ref{algo:algoGlobal} to deal with impulse control problems and shows very good performance on hedging with fixed transaction costs. This can be used to minimise a criteria which is a tradeoff between costs and a moment-based criteria. As we can also add constraints on the stopping times, instead of considering a penalty on the costs, one could also limit the total cost for each trajectory (by limiting the number of exercises).

==> inputs/abrege.tex <==
% TEX 7(ascii) bits
%
% ABREGE.tex
% LaTeX document
% Author: J.I. 
% Date  : Juillet 1996
%
% Raccourcis d'expressions tr\`es usit\'ees
%
% Derniere modif le 10-07-96
%

% Raccourci pour \XS
\def\XS{\xspace}

%%%%%%%%%%%%%%%%%%% Pour definir nouvelle commande de changement de taille
\RequirePackage{ifthen}
\RequirePackage{calc}

\newcommand{\taille}[1][\scad]{%
\ifthenelse{#1 = -5}{}{}%
\ifthenelse{#1 = -4}{\tiny}{}%
\ifthenelse{#1 = -3}{\scriptsize}{}%
\ifthenelse{#1 = -2}{\footnotesize}{}%
\ifthenelse{#1 = -1}{\small}{}%
\ifthenelse{#1 = 0}{\normalsize}{}%
\ifthenelse{#1 = 1}{\large}{}%
\ifthenelse{#1 = 2}{\Large}{}%
\ifthenelse{#1 = 3}{\LARGE}{}%
\ifthenelse{#1 = 4}{\huge}{}%
\ifthenelse{#1 = 5}{\Huge}{}}

\newboolean{@serif}
\setboolean{@serif}{true}
\def\scad{-5} % scadefaultsize

\newcounter{taille}
\newcommand{\sca}[2][\scad]{\setcounter{taille}{#1}%
  \ifthenelse{\boolean{@serif}}
  {{\taille[\thetaille]\textsc{#2}}}
  {\setcounter{taille}{\value{taille}-1}{\uppercase{\taille[\thetaille]#2}}}}

% Mise en commentaire rapide !
\def\rem#1{}                    % rem{bla bla bla}

% References automatiquement entre parenthese
\def\reff#1{\XS(\ref{#1})}
\def\refs#1{section~\ref{#1}}
\def\refS#1{Section~\ref{#1}}

\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}  
% Num?ro (pour biblio)
\def\numero{n?}
\def\Numero{N?}

% Majuscules
\def\UP#1{\uppercase{#1}}       % majuscules
\def\up#1{\uppercase{#1}}       % majuscules

% Liste des abreges
\def\adhoc{\textit{ad hoc}\XS}
\def\apost{\textit{a posteriori}\XS}
\def\Apost{\textit{A posteriori}\XS}
\def\APost{\textit{A Posteriori}\XS}
\def\post{\textit{posterior}\XS}
\def\Post{\textit{Posterior}\XS}
\def\afortio{\textit{a fortiori}\XS}
\def\Afortio{\textit{A fortiori}\XS}
\def\aprio{\textit{a priori}\XS}
\def\Aprio{\textit{A priori}\XS}
\def\Cad{C'est-\`a-dire\XS}
\def\cad{c'est-\`a-dire\XS}
\def\coeur{c{\oe}ur\XS}
\def\cf{\textit{cf.}\XS}
\def\cv{\textit{curriculum vit\ae}\XS}
\def\Cv{\textit{Curriculum vit\ae}\XS}
\def\CV{\textit{Curriculum Vit\ae}\XS}
\def\eg{\textit{e.g.,}\XS}
\def\etal{\textit{et al.}\XS}
\def\etc{\textit{etc}\XS}
\def\etcoll{{\textit et coll.}\XS}
\def\idem{\textit{idem}\XS}
\def\ie{\textit{i.e.,}\XS}
\def\IFF{\textit{if and only if}\XS}
\def\iid{i.i.d.\XS}
\def\infine{\textit{in fine}\XS}
\def\insit{\textit{in situ}\XS}
\def\inviv{\textit{in vivo}\XS}
\def\oeuvre{{\oe}uvre\XS}
\def\oeuvres{{\oe}uvres\XS}
\def\oeil{{\oe}il\XS}
\def\recto{\textit{recto}\XS}
\def\Toeplitz{T{\oe}plitz\XS}
\def\vav{vis-\`a-vis\XS}
\def\via{\textit{via}\XS}
\def\vic{\textit{vice-versa}\XS}
\def\verso{\textit{verso}\XS}
%\def\vitae{\textit{vit\ae}\XS}
\def\vs{\textit{vs}\XS}
\def\versus{\textit{versus}\XS}
\def\ssi{\textit{si et seulement si}\XS}
\def\strsen{\textit{stricto sensu}\XS}
\def\wrt{w.r.t.\XS}

\def\ier{$^{\text{\small er}}$\XS}
\def\iere{$^{\text{\small re}}$\XS}
\def\ieme{$^{\text{\small e}}$\XS}

\def\primo{\ensuremath{1^{\oD}}\XS}
\def\secundo{\ensuremath{2^{\oD}}\XS}
\def\tertio{\ensuremath{3^{\oD}}\XS}
\def\quatro{\ensuremath{4^{\oD}}\XS}


\newcommand{\art}[1][\scad]{\sca[#1]{art}\XS}
\newcommand{\cnd}[1][\scad]{\sca[#1]{cnd}\XS}
\newcommand{\ndt}[1][\scad]{\sca[#1]{ndt}\XS}
\newcommand{\gnc}[1][\scad]{\sca[#1]{gnc}\XS}
\newcommand{\mfa}[1][\scad]{\sca[#1]{mfa}\XS}
\newcommand{\map}[1][\scad]{\sca[#1]{map}\XS}

\newcommand{\icm}[1][\scad]{\sca[#1]{icm}\XS}
\newcommand{\icd}[1][\scad]{\sca[#1]{icd}\XS}
\newcommand{\rsb}[1][\scad]{\sca[#1]{rsb}\XS}
\newcommand{\snr}[1][\scad]{\sca[#1]{snr}\XS}

\newcommand{\dess}[1][\scad]{\sca[#1]{dess}\XS}
\newcommand{\dea}[1][\scad]{\sca[#1]{dea}\XS}
\newcommand{\deug}[1][\scad]{\sca[#1]{deug}\XS}
\newcommand{\deust}[1][\scad]{\sca[#1]{deust}\XS}
\newcommand{\iut}[1][\scad]{\sca[#1]{iut}\XS}
\newcommand{\iup}[1][\scad]{\sca[#1]{iup}\XS}

\newcommand{\eea}[1][\scad]{\sca[#1]{eea}\XS}
\def\EEA{\'Electronique \'Electrotechnique Automatique\XS}
\newcommand{\ats}[1][\scad]{\sca[#1]{ats}\XS}
\def\ATS{Automatique et Traitement du Signal\XS}

\newcommand{\te}[1][\scad]{\sca[#1]{te}\XS}
\def\TE{travaux d'?tudes\XS}
\newcommand{\td}[1][\scad]{\sca[#1]{td}\XS}
\def\TD{travaux dirig?s\XS}
\newcommand{\tp}[1][\scad]{\sca[#1]{tp}\XS}
\def\TP{travaux pratiques\XS}
%\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}
\def\TDAO{travaux dirig?s assist?s sur ordinateur\XS}
\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}
\def\ts{traitement du signal\XS}
\def\TS{Traitement du Signal\XS}

\newcommand{\gbm}[1][\scad]{\sca[#1]{gbm}\XS}
\newcommand{\irmf}[1][\scad]{\sca[#1]{irm-f}\XS}
\newcommand{\irm}[1][\scad]{\sca[#1]{irm}\XS}
\newcommand{\rmn}[1][\scad]{\sca[#1]{rmn}\XS}
\newcommand{\eeg}[1][\scad]{\sca[#1]{eeg}\XS}
\newcommand{\meg}[1][\scad]{\sca[#1]{meg}\XS}

\newcommand{\pc}[1][\scad]{\sca[#1]{pc}\XS}
% Operating Systemes 
\newcommand{\linux}[1][\scad]{\sca[#1]{Linux}\XS}
\newcommand{\unix}[1][\scad]{\sca[#1]{Unix}\XS}
\newcommand{\msdos}[1][\scad]{\sca[#1]{msdos}\XS}
\newcommand{\sunos}[1][\scad]{\sca[#1]{Sunos}\XS}
\newcommand{\hupux}[1][\scad]{\sca[#1]{hp-ux}\XS}
\newcommand{\vms}[1][\scad]{\sca[#1]{vms}\XS}
\newcommand{\solaris}[1][\scad]{\sca[#1]{Solaris}\XS}
\newcommand{\winnt}[1][\scad]{\sca[#1]{Windows-nt}\XS}
\newcommand{\vmware}[1][\scad]{\sca[#1]{vmware}\XS}
\newcommand{\win}[1][\scad]{\sca[#1]{Windows}\XS}

% Calcul scientifique
\newcommand{\labview}[1][\scad]{\sca[#1]{Labview}\XS}
\newcommand{\matlab}[1][\scad]{\sca[#1]{Matlab}\XS}
\newcommand{\maple}[1][\scad]{\sca[#1]{Maple}\XS}
\newcommand{\mathe}[1][\scad]{\sca[#1]{Mathematica}\XS}
\newcommand{\idl}[1][\scad]{\sca[#1]{Idl}\XS}

% langages
\newcommand{\cmex}[1][\scad]{\sca[#1]{Cmex}\XS}
\newcommand{\pascal}[1][\scad]{\sca[#1]{Pascal}\XS}
\newcommand{\java}[1][\scad]{\sca[#1]{Java}\XS}
\newcommand{\lisp}[1][\scad]{\sca[#1]{Lisp}\XS}
\newcommand{\forts}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 77}\XS}
\newcommand{\fortq}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 90}\XS}
\newcommand{\ada}[1][\scad]{\sca[#1]{Ada}\XS}
\newcommand{\eiffel}[1][\scad]{\sca[#1]{Eiffel}\XS}
\newcommand{\tcsh}[1][\scad]{\sca[#1]{tcsh}\XS}
\newcommand{\bash}[1][\scad]{\sca[#1]{bash}\XS}
\newcommand{\lgc}[1][\scad]{\sca[#1]{C}\XS}
\newcommand{\cpp}[1][\scad]{\sca[#1]{C}{\footnotesize ++}\XS}

\def\crec{charg? de recherches\XS}
\def\Crec{Charg? de recherches\XS}
\def\dr{directeur de recherches\XS}
\def\Dr{Directeur de recherches\XS}


% congres
\newcommand{\gretsi}[1][\scad]{\sca[#1]{gretsi}\XS}
\newcommand{\maxent}[1][\scad]{\sca[#1]{maxent}\XS}
\newcommand{\icip}[1][\scad]{\sca[#1]{icip}\XS}
\newcommand{\icassp}[1][\scad]{\sca[#1]{icassp}\XS}
\newcommand{\spie}[1][\scad]{\sca[#1]{spie}\XS}
\newcommand{\gdr}[1][\scad]{\sca[#1]{gdr--prc~isis}\XS}
\newcommand{\rfia}[1][\scad]{\sca[#1]{rfia}\XS}
\newcommand{\eusipco}[1][\scad]{\sca[#1]{eusipco}\XS}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ajout de famouss.tex
% modif le 25/5/2000 Phiphi
% GPInuts - Famous people - VIP
%
\newcommand{\beaunom}[4][0]{{\taille[#1]#2 \uppercase{#3}}%
{\sca[#1]{#4}}\XS}

%\newcommand{\MA}[1][\scad]{{\taille[#1]Marc \uppercase{A}}% 
%{\sca[#1]{llain}\XS}}
\newcommand{\MA}[1][\scad]{\beaunom[#1]{Marc}{A}{llain}}
\newcommand{\AB}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc}}
\newcommand{\ABF}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc~--~Fusco}}
\newcommand{\AC}[1][\scad]{\beaunom[#1]{Alain}{C}{oulais}}
\newcommand{\AH}[1][\scad]{\beaunom[#1]{Alain}{H}{erment}}
\newcommand{\AMD}[1][\scad]{\beaunom[#1]{Ali}{M}{ohammad--Djafari}}
\newcommand{\AR}[1][\scad]{\beaunom[#1]{Andrea}{R}{idolfi}}
\newcommand{\CH}[1][\scad]{\beaunom[#1]{Christian}{H}{einrich}}
\newcommand{\CS}[1][\scad]{\beaunom[#1]{Charles}{S}{oussen}}
\newcommand{\DLB}[1][\scad]{\beaunom[#1]{Denis}{L}{e Bihan}}
\newcommand{\FC}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{C}{hampagnat}}
\newcommand{\FL}[1][\scad]{\beaunom[#1]{Franck}{L}{etimonier}}
\newcommand{\FV}[1][\scad]{\beaunom[#1]{Francisco}{V}{arela}}
\newcommand{\FDU}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{D}{ublanchet}}
\newcommand{\GDE}[1][\scad]{\beaunom[#1]{Guy}{D}{emoment}}
\newcommand{\GLB}[1][\scad]{\beaunom[#1]{Guy Le}{B}{esnerais}}
\newcommand{\HC}[1][\scad]{\beaunom[#1]{Herv\'e}{C}{arfantan}}
\newcommand{\JFB}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{B}{ercher}}
\newcommand{\JFG}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{G}{iovannelli}}
\newcommand{\JFM}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{M}{angin}}
\newcommand{\JI}[1][\scad]{\beaunom[#1]{J\'er\^ome}{I}{dier}}
\newcommand{\JBP}[1][\scad]{\beaunom[#1]{Jean-Baptiste}{P}{oline}}
\newcommand{\MF}[1][\scad]{\beaunom[#1]{Marc}{F}{ayolle}}
\newcommand{\Mimi}[1][\scad]{\beaunom[#1]{Myriam}{F}{iani}}
\newcommand{\MN}[1][\scad]{\beaunom[#1]{Mila}{N}{ikolova}}
\newcommand{\PC}[1][\scad]{\beaunom[#1]{Philippe}{C}{iuciu}}
\newcommand{\LG}[1][\scad]{\beaunom[#1]{Line}{G}{arnero}}
\newcommand{\SB}[1][\scad]{\beaunom[#1]{St\'ephane}{B}{rette}}
\newcommand{\SBA}[1][\scad]{\beaunom[#1]{Sylvain}{B}{ailet}}
\newcommand{\RB}[1][\scad]{\beaunom[#1]{Redha}{B}{oubertakh}}
\newcommand{\TM}[1][\scad]{\beaunom[#1]{Thierry}{M}{artin}}
\newcommand{\VS}[1][\scad]{\beaunom[#1]{Vincent}{S}{amson}}
\newcommand{\YG}[1][\scad]{\beaunom[#1]{Yves}{G}{oussard}}
\newcommand{\KS}[1][\scad]{\beaunom[#1]{Ken}{S}{auer}}
\newcommand{\HS}[1][\scad]{\beaunom[#1]{Hichem}{S}{noussi}}

% Acronymes et raccourcis
%
\def\ATER{Attach\'e temporaire d'enseignement et de recherche}
\newcommand{\ater}[1][\scad]{\sca[#1]{ater}\xspace}
\def\ADDOC{Agir pour les Doctorants et les jeunes Docteurs\XS}
\newcommand{\addoc}[1][\scad]{\sca[#1]{addoc}\XS}

\def\CdO{Centre d'Orsay\XS}

\def\CEA{Commissariat ? l'\'Enegie Atomique\XS}
\newcommand{\cea}[1][\scad]{\sca[#1]{cea}\XS}
\newcommand{\dam}[1][\scad]{\sca[#1]{dam}\XS}
\def\DRM{D\'epartement de Recherche M\'edicale\XS}
\newcommand{\drm}[1][\scad]{\sca[#1]{drm}\XS}
\def\DSV{Direction des Sciences du Vivant\XS}
\newcommand{\dsv}[1][\scad]{\sca[#1]{dsv}\XS}
\newcommand{\leti}[1][\scad]{\sca[#1]{leti}\XS}
\def\SHFJ{Service Hospitalier Fr?d?ric Joliot\XS}
\newcommand{\shfj}[1][\scad]{\sca[#1]{shfj}\XS}
\def\UNAF{Unit\'e de Neuroimagerie Anatomo Foncxtionnelle\XS}
\newcommand{\unaf}[1][\scad]{\sca[#1]{unaf}\XS}


\newcommand{\chu}[1][\scad]{\sca[#1]{chu}\XS}
\def\CHU{Centre Hospitalier Universitaire\XS}
\def\salpe{Salp?tri?re\XS}
\def\hsalpe{H?pital de la Salp?tri?re\XS}
\def\pisalpe{Piti?-Salp?tri?re\XS}
\def\gpisalpe{Groupe Piti?-Salp?tri?re\XS}

\def\CNRS{Centre National de la Recherche Scientifique\XS}
\newcommand{\cnrs}[1][\scad]{\sca[#1]{cnrs}\XS}

\newcommand{\edf}[1][\scad]{\sca[#1]{edf}\XS}
\def\EDF{\'Electricit? de France\XS}

\def\ENSTA{\'Ecole Nationale Sup\'erieure de Techniques Avanc\'ees\XS}
\newcommand{\ensta}[1][\scad]{\sca[#1]{ensta}\XS}
\def\ESIEA{\'Ecole Sup?rieure d'Informatique \'Electronique Automatique\XS}
\newcommand{\esiea}[1][\scad]{\sca[#1]{esiea}\XS}
\newcommand{\ensea}[1][\scad]{\sca[#1]{ensea}\XS}


\def\GPI{Groupe Probl\`emes Inverses\XS}
\newcommand{\gpi}[1][\scad]{\sca[#1]{gpi}\XS}

\def\INSERM{Institut National pour la Sant\'e et la Recherche M\'edicale\XS}
\newcommand{\inserm}[1][\scad]{\sca[#1]{inserm}\XS}

\def\CNAM{Conservatoire National des Arts et M?tiers\XS}
\newcommand{\cnam}[1][\scad]{\sca[#1]{cnam}\XS}

\def\INRIA{Institut National de Recherche et Informatique et Automatique\XS}
\newcommand{\inria}[1][\scad]{\sca[#1]{inria}\XS}

\def\IAS{Institut d'Astrophysique Spatiale\XS}
\newcommand{\ias}[1][\scad]{\sca[#1]{ias}\XS}

\newcommand{\ipsn}[1][\scad]{\sca[#1]{ipsn}\XS}
\def\IPSN{Institut de Protection et de Suret? Nucl?aire\XS}

\def\LSS{Laboratoire des Signaux et Syst\`emes\XS}
\newcommand{\lss}[1][\scad]{\sca[#1]{l{\footnotesize 2}s}\XS}

\def\LIMSI{Laboratoire d'Informatique pour la M?canique et les Sciences de l'Ing?nieur\XS}
\newcommand{\limsi}[1][\scad]{\sca[#1]{limsi-cnrs}\XS}

\def\ONERA{Office National d'\'Etudes et de Recherches A\'erospatiales\XS}
\newcommand{\onera}[1][\scad]{\sca[#1]{on\'era}\XS}

\def\MDC{Ma\^\i tre de conf\'erences\XS}
\def\MDCs{Ma\^\i tres de conf\'erences\XS}
\newcommand{\mdc}[1][\scad]{\sca[#1]{mdc}\XS}

\newcommand{\UND}[1][\scad]{Universit? de Notre Dame, \sca[#1]{usa}\XS}

\def\UPS{Universit\'e Paris-Sud\XS}
\newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}
\newcommand{\upxi}[1][\scad]{\sca[#1]{upxi}\XS}

% Unites Thomson
\newcommand{\thomair}[1][\scad]{\sca[#1]{Thomson-csf Airsys}\XS}
\newcommand{\oscar}[1][\scad]{\sca[#1]{Oscar}\XS}
\newcommand{\thomrcm}[1][\scad]{\sca[#1]{Thomson-rcm}\XS}

% Unite propre de recherche
\newcommand{\upr}[1][\scad]{\sca[#1]{upr}\XS}
% LENA, lena upr640,...
\newcommand{\uprlen}[1][\scad]{\sca[#1]{upr}{\footnotesize 640}\XS}
\def\LENA{Laboratoire d'Enc?phalographie et de Neurophysiologie Appliqu?e\XS}
\newcommand{\lena}[1][\scad]{\sca[#1]{lena}\XS}
% Nous
\def\GsY{Gif--sur--Yvette\XS}
\newcommand{\ESE}[1][\scad]{\sca[#1]{sup\'elec}\XS}

\def\adrshort{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex\XS}
%\def\adresse{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
\newcommand{\hiercea}[1][\scad]{\dsv[#1]/\drm[#1]/\shfj[#1]\XS}

\newcommand{\adresse}[1][\scad]{\ESE[#1], Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
\newcommand{\adresscea}[1][\scad]{4 Place du G?n?ral Leclerc, 91406 Orsay Cedex, France\XS}
\newcommand{\tutelle}[1][\scad]{\cnrs[#1]~--~\ESE[#1]~--~\ups[#1]}
%\newcommand{\tutelle}[1][\scad]{\sca[#1]{Cnrs~--~Sup\'elec~--~Ups}}
\def\ALSS{\LSS~(\tutelle)\\\adresse}
\def\ALSSun{\LSS (\tutelle) \adresse}
%


% ---------------------------------------------------- 
% Modele d'en-tete par A. Mohammad-Djafari et J. Idier 
% ---------------------------------------------------- 
%
\def\helvnormal#1{{\fontfamily{phv}\fontsize{11}{14pt}\selectfont #1}}
\def\helvfoot  #1{{\fontfamily{phv}\fontsize{9}{14pt} \selectfont #1}}
\def\helvscript#1{{\fontfamily{phv}\fontsize{8}{14pt} \selectfont #1}}
%
\newcommand{\entete}[5][Nom.Pr\'enom]{
%%%%%%\def\entete#1#2#3#4#5{%
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Sup?lec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique          \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYST\`EMES}}\\%
\helvfoot{Unit\'e mixte de recherche n$^{\rm o}$ 8506\\%
Sup\'elec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
T\'el\'ephone\,: 01 69 85 17 12 --- 
T\'el\'ecopie\,: 01 69 85 17 65 --- 
Courriel\,: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{V/R\'ef.\,: #2} & \helvscript{\sca[-3]{Gif}, le} #5\\%
\helvscript{N/R\'ef.\,: #3} \\%
\helvscript{Objet\,: #4}%
\end{tabular}
} 

\newcommand{\inhead}[5][Name.Surname]{
%%%%%%\def\entete#1#2#3#4#5{%
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Sup?lec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique  \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYST\`EMES}}\\%
\helvfoot{Unit\'e mixte de recherche n$^{\rm o}$ 8506\\%
Sup\'elec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
Telephone: 01 69 85 17 12 --- 
Fax: 01 69 85 17 65 --- 
E-mail: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{Y/Ref.: #2} & \helvscript{\sca[-3]{Gif}, } #5\\%
\helvscript{O/Ref.: #3} \\%
\helvscript{Subject: #4}%
\end{tabular}
} 



==> inputs/alphabet.tex <==
% Document LaTeX        Auteur : Guy Le Besnerais       Date : 25/05/94
% Modification : J.-F. Gio      (15/09/95)
%                               J.I. (format Latex 2e, taille adaptative 22/03/99)
%                                    (fonte blackboard 27/08/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace, amsmath, bbm)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}
\RequirePackage{bbm}
\RequirePackage{oldgerm}		% 04.06.2003   Pour les alphabet Gauthiques

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}

% ALPHABET GRAS et Chapeau
\def\Abh{\hat{{\sbm{A}}}\XS}  \def\abh{\hat{{\sbm{a}}}\XS}
\def\Bbh{\hat{{\sbm{B}}}\XS}  \def\bbh{\hat{{\sbm{b}}}\XS}
\def\Cbh{\hat{{\sbm{C}}}\XS}  \def\cbh{\hat{{\sbm{c}}}\XS}
\def\Dbh{\hat{{\sbm{D}}}\XS}  \def\dbh{\hat{{\sbm{d}}}\XS}
\def\Ebh{\hat{{\sbm{E}}}\XS}  \def\ebh{\hat{{\sbm{e}}}\XS}
\def\Fbh{\hat{{\sbm{F}}}\XS}  \def\fbh{\hat{{\sbm{f}}}\XS}
\def\Gbh{\hat{{\sbm{G}}}\XS}  \def\gbh{\hat{{\sbm{g}}}\XS}
\def\Hbh{\hat{{\sbm{H}}}\XS}  \def\hbh{\hat{{\sbm{h}}}\XS}
\def\Ibh{\hat{{\sbm{I}}}\XS}  \def\ibh{\hat{{\sbm{i}}}\XS}
\def\Jbh{\hat{{\sbm{J}}}\XS}  \def\jbh{\hat{{\sbm{j}}}\XS}
\def\Kbh{\hat{{\sbm{K}}}\XS}  \def\kbh{\hat{{\sbm{k}}}\XS}
\def\Lbh{\hat{{\sbm{L}}}\XS}  \def\lbh{\hat{{\sbm{l}}}\XS}
\def\Mbh{\hat{{\sbm{M}}}\XS}  \def\mbh{\hat{{\sbm{m}}}\XS}
\def\Nbh{\hat{{\sbm{N}}}\XS}  \def\nbh{\hat{{\sbm{n}}}\XS}
\def\Obh{\hat{{\sbm{O}}}\XS}  \def\obh{\hat{{\sbm{o}}}\XS}
\def\Pbh{\hat{{\sbm{P}}}\XS}  \def\pbh{\hat{{\sbm{p}}}\XS}
\def\Qbh{\hat{{\sbm{Q}}}\XS}  \def\qbh{\hat{{\sbm{q}}}\XS}
\def\Rbh{\hat{{\sbm{R}}}\XS}  \def\rbh{\hat{{\sbm{r}}}\XS}
\def\Sbh{\hat{{\sbm{S}}}\XS}  \def\sbh{\hat{{\sbm{s}}}\XS}
\def\Tbh{\hat{{\sbm{T}}}\XS}  \def\tbh{\hat{{\sbm{t}}}\XS}
\def\Ubh{\hat{{\sbm{U}}}\XS}  \def\ubh{\hat{{\sbm{u}}}\XS}
\def\Vbh{\hat{{\sbm{V}}}\XS}  \def\vbh{\hat{{\sbm{v}}}\XS}
\def\Wbh{\hat{{\sbm{W}}}\XS}  \def\wbh{\hat{{\sbm{w}}}\XS}
\def\Xbh{\hat{{\sbm{X}}}\XS}  \def\xbh{\hat{{\sbm{x}}}\XS}
\def\Ybh{\hat{{\sbm{Y}}}\XS}  \def\ybh{\hat{{\sbm{y}}}\XS}
\def\Zbh{\hat{{\sbm{Z}}}\XS}  \def\zbh{\hat{{\sbm{z}}}\XS}

\def\alphabh      {\hat{{\sbmm{\alpha}}}\XS}
\def\betabh       {\hat{{\sbmm{\beta}}}\XS}
\def\gammabh      {\hat{{\sbmm{\gamma}}}\XS}      \def\Gammabh    {\hat{{\sbmm{\Gamma}}}\XS}
\def\deltabh      {\hat{{\sbmm{\delta}}}\XS}      \def\Deltabh    {\hat{{\sbmm{\Delta}}}\XS}
\def\epsilonbh    {\hat{{\sbmm{\epsilon}}}\XS}
\def\varepsilonbh {\hat{{\sbmm{\varepsilon}}}\XS}
\def\etabh        {\hat{{\sbmm{\eta}}}\XS}
\def\thetabh      {\hat{{\sbmm{\theta}}}\XS}      \def\Thetabh    {\hat{{\sbmm{\Theta}}}\XS}
\def\varthetabh   {\hat{{\sbmm{\vartheta}}}\XS}
\def\iotabh       {\hat{{\sbmm{\iota}}}\XS}
\def\kappabh      {\hat{{\sbmm{\kappa}}}\XS}
\def\varkappabh   {\hat{{\sbmm{\varkappa}}}\XS}
\def\lambdabh     {\hat{{\sbmm{\lambda}}}\XS}     \def\Lambdabh   {\hat{{\sbmm{\Lambda}}}\XS}
\def\mubh         {\hat{{\sbmm{\mu}}}\XS}
\def\nubh         {\hat{{\sbmm{\nu}}}\XS}
\def\xibh         {\hat{{\sbmm{\xi}}}\XS}         \def\Xibh       {\hat{{\sbmm{\Xi}}}\XS}
\def\pibh         {\hat{{\sbmm{\pi}}}\XS}         \def\Pibh       {\hat{{\sbmm{\Pi}}}\XS}
\def\varpibh      {\hat{{\sbmm{\varpi}}}\XS}
\def\rhobh        {\hat{{\sbmm{\rho}}}\XS}
\def\varrhobh     {\hat{{\sbmm{\varrho}}}\XS}
\def\sigmabh      {\hat{{\sbmm{\sigma}}}\XS}      \def\Sigmabh    {\hat{{\sbmm{\Sigma}}}\XS}
\def\varsigmabh   {\hat{{\sbmm{\varsigma}}}\XS}   \def\Varsigmabh {\hat{{\sbmm{\Varsigma}}}\XS}
\def\phibh        {\hat{{\sbmm{\phi}}}\XS}        \def\Phibh      {\hat{{\sbmm{\Phi}}}\XS}
\def\varphibh     {\hat{{\sbmm{\varphi}}}\XS}
\def\chibh        {\hat{{\sbmm{\chi}}}\XS}
\def\psibh        {\hat{{\sbmm{\psi}}}\XS}        \def\Psibh      {\hat{{\sbmm{\Psi}}}\XS}
\def\omegabh      {\hat{{\sbmm{\omega}}}\XS}      \def\Omegabh    {\hat{{\sbmm{\Omega}}}\XS}
\def\taubh        {\hat{{\sbmm{\tau}}}\XS}
\def\upsilonbh    {\hat{{\sbmm{\upsilon}}}\XS}   \def\Upsilonbh  {\hat{{\sbmm{\Upsilon}}}\XS}
\def\zetabh       {\hat{{\sbmm{\zeta}}}\XS}





% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}

% ALPHABET GAUTHIQUES  04.06.2003  M.M. ICHIR

\def\Ag{{\textgoth{A}}\XS}  \def\ag{{\textgoth{a}}\XS}
\def\Bg{{\textgoth{B}}\XS}  \def\bg{{\textgoth{b}}\XS}
\def\Cg{{\textgoth{C}}\XS}  \def\cg{{\textgoth{c}}\XS}
\def\Dg{{\textgoth{D}}\XS}  \def\dg{{\textgoth{d}}\XS}
\def\Eg{{\textgoth{E}}\XS}  \def\eg{{\textgoth{e}}\XS}
\def\Fg{{\textgoth{F}}\XS}  \def\fg{{\textgoth{f}}\XS}
\def\Gg{{\textgoth{G}}\XS}  \def\gg{{\textgoth{g}}\XS}
\def\Hg{{\textgoth{H}}\XS}  \def\hg{{\textgoth{h}}\XS}
\def\Ig{{\textgoth{I}}\XS}  \def\ig{{\textgoth{i}}\XS}
\def\Jg{{\textgoth{J}}\XS}  \def\jg{{\textgoth{j}}\XS}
\def\Kg{{\textgoth{K}}\XS}  \def\kg{{\textgoth{k}}\XS}
\def\Lg{{\textgoth{L}}\XS}  \def\lg{{\textgoth{l}}\XS}
\def\Mg{{\textgoth{M}}\XS}  \def\mg{{\textgoth{m}}\XS}
\def\Ng{{\textgoth{N}}\XS}  \def\ng{{\textgoth{n}}\XS}
\def\Og{{\textgoth{O}}\XS}  \def\og{{\textgoth{o}}\XS}
\def\Pg{{\textgoth{P}}\XS}  \def\pg{{\textgoth{p}}\XS}
\def\Qg{{\textgoth{Q}}\XS}  \def\qg{{\textgoth{q}}\XS}
\def\Rg{{\textgoth{R}}\XS}  \def\rg{{\textgoth{r}}\XS}
\def\Sg{{\textgoth{S}}\XS}  \def\sg{{\textgoth{s}}\XS}
\def\Tg{{\textgoth{T}}\XS}  \def\tg{{\textgoth{t}}\XS}
\def\Ug{{\textgoth{U}}\XS}  \def\ug{{\textgoth{u}}\XS}
\def\Vg{{\textgoth{V}}\XS}  \def\vg{{\textgoth{v}}\XS}
\def\Wg{{\textgoth{W}}\XS}  \def\wg{{\textgoth{w}}\XS}
\def\Xg{{\textgoth{X}}\XS}  \def\xg{{\textgoth{x}}\XS}
\def\Yg{{\textgoth{Y}}\XS}  \def\yg{{\textgoth{y}}\XS}
\def\Zg{{\textgoth{Z}}\XS}  \def\zg{{\textgoth{z}}\XS}

